From Form(s) to Meaning: Probing the Semantic Depths of Language Models Using Multisense Consistency

The staggering pace with which the capabilities of large language models (LLMs) are increasing, as measured by a range of commonly used natural language understanding (NLU) benchmarks, raises many questions regarding what "understanding" means for a language model and how it compares to human understanding. This is especially true since many LLMs are exclusively trained on text, casting doubt on whether their stellar benchmark performances are reflective of a true understanding of the problems represented by these benchmarks, or whether LLMs simply excel at uttering textual forms that correlate with what someone who understands the problem would say. In this philosophically inspired work, we aim to create some separation between form and meaning, with a series of tests that leverage the idea that world understanding should be consistent across presentational modes - inspired by Fregean senses - of the same meaning. Specifically, we focus on consistency across languages as well as paraphrases. Taking GPT-3.5 as our object of study, we evaluate multisense consistency across five different languages and various tasks. We start the evaluation in a controlled setting, asking the model for simple facts, and then proceed with an evaluation on four popular NLU benchmarks. We find that the model's multisense consistency is lacking and run several follow-up analyses to verify that this lack of consistency is due to a sense-dependent task understanding. We conclude that, in this aspect, the understanding of LLMs is still quite far from being consistent and human-like, and deliberate on how this impacts their utility in the context of learning about human language and understanding.

==> tables/simple_facts_templates_old.tex <==
\begin{table}[ht]
\caption{Templates for the \textsc{simple facts} datasets. In each template, we replaced the mask(s) with an example datapoint.
Replacements are indicated in bold.}\label{tab:templates}
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|l|l}
\toprule
dataset & subtask & template / example \\
\midrule
\multirow{3}{*}{\small\textsc{elements}}     &  \small \textsc{from-element}     &   \small ``What is the atomic number of the chemical element \textbf{He}?'' \\
\cline{2-3}
                                            &   \small \textsc{from-position}   &   \small ``What is the atomic number of the chemical element \\
                                            &                                   &   \small  in period \textbf{5} and group \textbf{7}?'' \\
\midrule
\multirow{2}{*}{\small\textsc{olympics}}    &   \small \textsc{100m}            &   \small ``Who won the \textbf{gold} medal in the \textbf{men's} 100 meters at the \\
                                            &                                   &   \small  \textbf{2000} Summer Olympics?'' \\
\cline{2-3}
                                            &   \small \textsc{downhill}        &   \small ``Who won the \textbf{bronze} medal in the \textbf{women's} downhill \\
                                            &                                   &   \small   competition at the \textbf{1976} Winter Olympics?'' \\
\midrule
\multirow{5}{*}{\small\textsc{writers}}     &  \small \textsc{english}        &   \small ``In what year was the writer \textbf{Allen Ginsberg} born?'' \\
\cline{2-3}
                                            &  \small \textsc{german}         &   \small ``In what year was the writer \textbf{Friedrich Schiller} born?'' \\
\cline{2-3}
                                            &  \small \textsc{italian}        &   \small ``In what year was the writer \textbf{Manuela Campanelli} born?'' \\
\cline{2-3}
                                            &  \small \textsc{dutch}          &   \small ``In what year was the writer \textbf{Betje Wolff} born?'' \\
\cline{2-3}
                                            &  \small \textsc{swedish}        &   \small ``In what year was the writer \textbf{Astrid Lindgren} born?'' \\
\midrule
\multirow{5}{*}{\small\textsc{companies}}       &  \small\textsc{american}  &   \small ``In what city does \textbf{Walmart Inc.} have its headquarters?'' \\
\cline{2-3}
                                                &  \small \textsc{german}   &   \small ``In what city does \textbf{Volkswagen AG} have its headquarters?'' \\
\cline{2-3}
                                                &  \small \textsc{italian}  &   \small ``In what city does \textbf{Webuild S.p.A.} have its headquarters?'' \\
\cline{2-3}
                                                &  \small\textsc{dutch}     &   \small ``In what city does \textbf{Airbus SE} have its headquarters?'' \\
\cline{2-3}
                                                &  \small \textsc{swedish}  &   \small ``In what city does \textbf{SEB Group} have its headquarters?'' \\
\midrule
\small\textsc{arithmetics}                      & \small\textsc{addition}  &   \small ``What is \textbf{three hundred seventy-five} plus \textbf{twenty-three}?''\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

